A Dimension-Independent discriminant between distributions

Henze-Penrose divergence is a non-parametric divergence measure that can be used to estimate a bound on the Bayes error in a binary classification problem. In this paper, we show that a cross-match statistic based on optimal weighted matching can be used to directly estimate Henze-Penrose divergence. Unlike an earlier approach based on the Friedman-Rafsky minimal spanning tree statistic, the proposed method is dimension-independent. The new approach is evaluated using simulation and applied to real datasets to obtain Bayes error estimates.

==> HP-divergence.tex <==
\section{Binary Classification}
\label{sec:BER}

Examples of discrete classification algorithm include the discrete histogram rule, {\bf Cite}, the maximum-mean-accuracy algorithm {\bf Cite}, and many other examples of discrete rules used in Data Mining {\bf Cite}. Among these, the discrete histogram rule is by far the most used one in practice because of its simplicity as majority voting over the bins, and also because of the plug-in rule for approximating the optimal Bayes classifier. \\
\def\BX{\mathbf{X}}
\def\BY{\mathbf{Y}}
\def\bx{\mathbf{x}}
\def\R{\mathcal{R}}
\def\diy{\displaystyle}
Let discrete values $\bx_1,\bx_2,...,\bx_N$ in $\R^d$ be realization of random vector $\BX$ with the class label  variable $Y\in\{0,1\}$ with probabilities $c_0=P(Y=0)$ and $c_1=P(Y=1)$, such that $c_0+c_1=1$. Denote $p_0(\bx_i)=p(\BX=\bx_i|Y=0)$ and $p_1(\bx_i)=p(\BX=\bx_i|Y=1)$, $\sum\limits_{i=1}^n p_0(\bx_i)=\sum\limits_{i=1}^N p_1(\bx_i)=1$. Through Bayes theorem, these model parameters determine the posterior probabilities, 
$$P(Y=0|\BX=\bx_i)=\diy\frac{c_0p_0(\bx_i)}{c_0p_0(\bx_i)+c_1p_1(\bx_i)},$$
and $P(Y=1|\BX=\bx_i)=1-P(Y=0|\BX=\bx_i)$. The Bayes error rate (the expected risk) is given by
\begin{equation}
\epsilon=\diy\sum\limits_{i=1}^N \min\big\{c_0p_0(\bx_i),c_1p_1(\bx_i)\big\}.
\end{equation}
Equivalently for sets $A_0=\{x_i:c_0p_0(\bx_i)\geq c_1p_1(\bx_i)\}$ and $A_1=\{x_i:c_0p_0(\bx_i)\leq c_1p_1(\bx_i)\}$:
\begin{equation}\label{BER}
\epsilon=\diy\sum\limits_{A_0}c_0p_0(\bx_i)+\sum\limits_{A_1}c_1p_1(\bx_i).
\end{equation}
Following arguments in \cite{BWHS}, we can bound (\ref{BER}) by 
\begin{equation}
\diy\frac{1}{2}-\frac{1}{2}\sqrt{H_c(p_0,p_1)}\leq \epsilon\leq \frac{1}{2}-\frac{1}{2}H_c(p_0,p_1),
\end{equation}
where
$H_c(p_0,p_1)=1-4c_0c_1\diy\sum\limits_{i=1}^N \frac{p_0(\bx_i)p_1(\bx_i)}{c_0p_0(\bx_i)+c_1p_1(\bx_i)}.$



